Monitoring Fidelity of Online Reinforcement Learning Algorithms in Clinical Trials

Online reinforcement learning (RL) algorithms offer great potential for personalizing treatment for participants in clinical trials. However, deploying an online, autonomous algorithm in the high-stakes healthcare setting makes quality control and data quality especially difficult to achieve. This paper proposes algorithm fidelity as a critical requirement for deploying online RL algorithms in clinical trials. It emphasizes the responsibility of the algorithm to (1) safeguard participants and (2) preserve the scientific utility of the data for post-trial analyses. We also present a framework for pre-deployment planning and real-time monitoring to help algorithm developers and clinical researchers ensure algorithm fidelity. To illustrate our framework's practical application, we present real-world examples from the Oralytics clinical trial. Since Spring 2023, this trial successfully deployed an autonomous, online RL algorithm to personalize behavioral interventions for participants at risk for dental disease.

==> related_works.tex <==
\subsection{Literature on AI in Clinical Trials}

Two big things they talk about: 1) quality control (validtion, monitoring, reproducibility), and 2) data excellence (reporting, auditing, replicability of study). It's much more challenging for us because of the online nature of our algorithm.

Key Contributions Of Our Paper:
\begin{itemize}
    \item Detecting unique issues of an online algorithm in real-time (e.g., patient dosage beyond networking or system-level issues).
    \item Online property of algorithm produces the need for real-time monitoring (most people consider offline batch training).
    \item Most people talk about monitoring the deployment of the algorithm with a fixed policy. But not necessarily the \textit{fidelity} algorithm. Unintended negative consequences can affect patient experience during the study because of the online nature of the algorithm.
\end{itemize}

\paragraph{Types of papers in literature}
\begin{itemize}
    \item AI Quality Control: Considerations when designing, deploying, and monitoring AI models for health care and other high-stakes settings. Auditing.
    \alt{We are different because quality control is much harder when running and online algorithm. The online property of the algorithm produces the need for real-time monitoring (most people consider offline batch training). Autonomous updating.}
    \item Data reporting,  reproducibility, and data excellence in clinical trials \kwz{We are different because need to be able to reproduce the algorithm itself which has randomness and is updating. What does data excellence mean in the online decision making setting in clinical trials.}
\end{itemize}

\paragraph{Summary of papers:}
\begin{itemize}
    \item \bo{Artificial intelligence, bias and clinical safety.} Talk about training and deployment of AI models for healthcare (rather than algorithms that learn online). They discuss issues like distributional shift, explainability, unsafe failure modes. Short term, medium term, long term considerations \kwz{Focus is on potential unintended consequences (bias, failure modes, distribution shift) of deploying AI. Esp for supervised learning.}
    \alt{We contribute a framework for monitoring an \textit{online} algorithm: ``ML systems that are very frequently updated, and particularly those that continuously learn". This contributes trust towards clinical safety.}
    \item \bo{Reporting guidelines for clinical trial reports for interventions involving artificial intelligence: the CONSORT-AI extension.} Checklist for what to report about AI algorithms in clinical trials (versus clinical trials not using AI algorithms). For example, which version of algorithm used, how input data acquired, data quality, etc. \kwz{checklists for enhancing reproducibility and scientific validity} \alt{They mention reporting which version of the algorithm was used. We go into more detail and mention this doesn't just include the software version but also the policy that was used. Do they also mention the importance of reproducing the algorithm? Just knowing the version sometimes is not enough.}
    \item \bo{Artificial intelligence in dental research: Checklist for authors, reviewers, readers.} Study design, Data, Sampling, Data Protection, Missing data Data Processing, Reference Test, Sample Size, Model, Model parameters Training, Justify the best- performing model, Evaluation, Uncertainty Explainability Results \kwz{checklists for enhancing reproducibility and scientific validity}
    \item \bo{Artificial intelligence to enhance clinical value across the spectrum of cardiovascular healthcare.} Following a clear research hypothesis, an AI-based workflow begins with data selec- tion and pre-processing prior to analysis, with the type of data (structured, semi-structured, or unstructured) determining what type of pre-pro- cessing steps and machine-learning algorithms are required. Algorithmic and data validation should be performed to ensure the robustness of the chosen methodology, followed by an objective evaluation of performance. Seven case studies are provided to highlight the wide variety of data modalities and clinical questions that can benefit from modern AI techniques, with a focus on applying them to cardiovascular disease management. \kwz{AI workflow from data to training to deployment. A lot of focus is on supervised or unsupervised learning methods, rather than online algorithms.}
    \item \bo{Concrete Problems in AI Safety.} he problem of accidents in machine learning systems, defined as unintended and harmful behavior that may emerge from poor design of real-world AI systems. We present a list of five practical research problems related to accident risk, categorized according to whether the problem originates from having the wrong objective function (“avoiding side effects” and “avoiding reward hacking”), an objective function that is too expensive to evaluate frequently (“scalable supervision”), or undesirable behavior during the learning process (“safe exploration” and “distributional shift”). \kwz{Awareness of potential unintended consequences of AI deployment.}
    \item \bo{“Everyone wants to do the model work, not the data work”: Data Cascades in High-Stakes AI.} Data Cascades: compounding events causing negative, downstream efects from data issues, result- ing in technical debt4 over time. In our study, data cascades were widely prevalent: 92\% of AI practitioners reported experiencing one or more, and 45.3\% reported two or more cascades in a given project. Data cascades often resulted from applying conventional AI practices that undervalued data quality.
    \alt{highlights how poor data quality or undervaluing data in high-stakes domain have out-sized effects on living beings} \alt{Authors also mentioned that high-stakes AI often combines two or more disciplines. Challenge: greater collaboration. One example this comes up in Oralytics is we have to communicate to and have a contract with all systems on the data they provide and are saving. For example, main controller didn't know they needed to save the actual prompt of messages that are scheduled.} \alt{``Production iw the process of deploying systems `live', with a need to keep systems running smoothly and scaling efficiently."} \alt{Our paper: obtaining data excellence in the online RL clinical trial setting.}
    \item \bo{Ideal algorithms in healthcare: Explainable, dynamic, precise, autonomous, fair, and reproducible.} explainable (convey the relative importance of features in determining outputs), dynamic (capture temporal changes in physiologic signals and clinical events), precise (use high-resolution, multimodal data and aptly complex architecture), autonomous (learn with minimal supervision and execute without human input), fair (evaluate and mitigate implicit bias and social inequity), and reproducible (validated externally and prospectively and shared with academic communities). \kwz{importance of data quality and curation in real world deployments}
    \item \bo{ML4H Auditing: From Paper to Practice.} However, their transla- tion into medical practice is often ham- pered by a lack of careful evaluation in different settings. Efforts have started worldwide to establish guidelines for evaluating machine learning for health (ML4H) tools, highlighting the neces- sity to evaluate models for bias, inter- pretability, robustness, and possible fail- ure modes. However, testing and adopt- ing these guidelines in practice remains an open challenge. In this work, we tar- get the paper-to-practice gap by apply- ing an ML4H audit framework proposed by the ITU/WHO Focus Group on Arti- ficial Intelligence for Health (FG-AI4H) to three use cases: diagnostic prediction of diabetic retinopathy, diagnostic pre- diction of Alzheimer’s disease, and cyto- morphologic classification for leukemia diagnostics. The assessment comprises dimensions such as bias, interpretability, and robustness. \kwz{ideal qualities of algorithms for healthcare}
    \item \bo{Machine Learning for Health: Algorithm Auditing and Quality Control.} 
    the deployment of machine learning for health (ML4H) tools into real-world applications has been slow because existing approval pro- cesses [6] may not account for the particular failure modes and risks that accompany (ML) technology. In order to overcome this hurdle, we envision a frame- work of algorithm auditing and quality control that provides a path towards the effective and reliable application of ML systems in healthcare. \alt{Their updates are manual, between-trial updates.
    We are dealing with autonomous, real-time, within-trial updates.}
    \alt{Deployment and Monitoring look different for us. Even how you validate also looks different for us.}
    \begin{itemize}
        \item The typical ML product life cycle goes through stages of planning, development, validation and, potentially, deployment under appropriate monitoring (see Fig. 1B). Feedback loops between stages, for example from product validation back to development, are commonplace.
        \item An audit entails a detailed assessment of an ML4H tool at one or more of the ML life cycle steps. It can be carried out to anticipate, monitor, or retrospectively review operations of the tool. The audit output should consist of a comprehensive standardized report that can be used by different stakeholders to efficiently communicate the tool’s strengths and limitations
        \item \bo{Facet 1: technical validation} application of data and ML model quality assessment methods to detect possible failure modes in the model’s behavior. These include model-oriented metrics, such as predictive performance, robustness, interpretability, disparity or uncertainty, but also data oriented metrics related to sample size determination, sparseness, bias, distribution mismatch and label quality
        \item \bo{Facet 2: Clinical Evaluation} o analyse whether there is sufficient clinical evidence to confirm compliance with relevant essential requirements for safety and performance when using the device according to the manufacturer’s instructions for use
        \item \bo{Facet 3: Regulatory Assessment}
        \item \bo{Life cycle: plan, develop, validate, deploy and monitor}
    \end{itemize}
    \kwz{Focus a lot on supervised learning / rather than RL alg considerations. }
    \item \bo{Randomized Clinical Trials of Machine Learning Interventions in Health Care.} systematically examine the design, reporting standards, risk of bias, and inclusivity of RCTs for medical machine learning interventions.  Common reasons for nonadherence were not assessing poor-quality or unavailable input data (38 trials [93\%]), not analyzing performance errors (38 [93\%]), and not including a statement regarding code or algorithm availability (37 [90\%]). Overall risk of bias was high in 7 trials (17\%). Of 11 trials (27\%) that reported race and ethnicity data, the median proportion of participants from underrepresented minority groups was 21\% (range, 0\%-51\%). \kwz{Reasons behind not following clnical trial reporting guidelines/checklists. Reasons included not analyzing performance errors, not assessing input data, not including statement on algorithm availability / code.} 
    
    \item \bo{Guidelines for clinical trial protocols for interventions involving artificial intelligence: the SPIRIT-AI extension.}  The SPIRIT-AI extension includes 15 new items that were considered sufficiently important for clinical trial protocols of AI interventions. These new items should be routinely reported in addition to the core SPIRIT 2013 items. SPIRIT-AI recom- mends that investigators provide clear descriptions of the AI intervention, including instructions and skills required for use, the setting in which the AI intervention will be integrated, considerations for the handling of input and output data, the human–AI interaction and analysis of error cases. SPIRIT-AI will help promote transparency and completeness for clinical trial protocols for AI interventions. Its use will assist editors and peer reviewers, as well as the general readership, to understand, interpret and critically appraise the design and risk of bias for a planned clinical trial. \kwz{Similar to CONSORT-AI paper.}
\end{itemize}
